DeltaScience: Benchmarking AI Agents on Real Scientific Problems

AI agents are moving from static recall toward autonomous scientific workflows, yet most benchmarks test isolated QA or code snippets and cannot verify whether deliverables pass scientific acceptance. We introduce DeltaScience, an open evaluation platform for large models and AI agents in real scientific scenarios, dedicated to connecting frontier scientific discovery with real-world industrial R&D and testing AI scientific capability on problems that truly matter, turning capability gains into retestable scientific increments ($\delta$). DeltaScience uses a three-layer decoupled governance architecture: the non-profit DeltaScience Benchmark sets acceptance standards and versioned releases; Playground runs open task submissions, authoring competitions, and incentives; and Bohrium provides isolated sandboxes and compute infrastructure. DeltaScience v1.0 comprises 65 private tasks across 7 discipline groups, 35 subfields, and 4 task types (44.6% cross-group). Eleven versioned Model + Harness configurations run five isolated trials per task (3,575 runs), yielding six findings: (1) GPT-6.2 Astra + Codex leads at 61.3 (95% CI [51.3, 70.6]), ahead of GPT-6.2 Sol + Codex (56.0), Qwen4-Max + Qoder (44.0), Kimi K3.1 Pro + Kimi Code (40.5), and HY4 + DSH (38.3), with 45/55 pairs separated; (2) reliability lags ceiling--even #1 drops from pass@5 = 60.0% to pass^5 = 49.2%, and 61.1% of cells never pass; (3) task difficulty explains 52.3% of variance, while swapping the harness on HY4 (+11.0, [+6.7, +15.4]) outweighs swapping models; (4) inter-agent correlation averages 0.60, while Best-of-11 Oracle (69.6, +8.4) shows complementarity alongside 6 unsolved tasks; (5) runtime correlates negatively with accuracy ($\rho = -0.56$); and (6) Qwen4-Max + Qoder (41.8) leads GPT-6.2 (34.5--36.4) on Tool-Use & Planning.

==> generated/stats_zh.tex <==
% Auto-generated by scripts/generate_report_data.py -- Chinese-only macros
\newcommand{\DSTopOutcomeTagZH}{靶点选择性}


==> generated/tab_composition_zh.tex <==
\begin{tabularx}{\linewidth}{@{}l r X@{}}
\toprule
学科大类 & 覆盖题数 & 包含的细分类别（共 35 个） \\
\midrule
化学 & 24 & 药物化学（17）、有机化学（13）、化学信息学（5）、计算化学（4）、化学生物学（2）、分子光谱（2）、催化与电化学（1）、分析化学（1） \\
物理学 & 22 & 量子计算（8）、聚变与等离子体（5）、凝聚态物理（5）、统计物理（2）、原子分子物理（1）、生物物理（1） \\
生命科学 & 21 & 生物组学（13）、结构生物学（7）、生物信息学（5）、免疫与炎症（3）、肿瘤生物学（3）、干细胞与衰老（2） \\
数学与计算机 & 11 & 算法设计（4）、代数与组合（3）、运筹学（3）、机器学习（3）、控制理论（1）、编码理论（1）、计算数学（1） \\
材料科学 & 9 & 计算材料（5）、表面与纳米材料（3）、材料设计（1）、材料力学（1） \\
工程科学 & 6 & 工程设计（4）、流体力学（2）、传热（1） \\
地球科学 & 1 & 地球物理（1） \\
\bottomrule
\end{tabularx}


==> generated/tab_groupmatrix_en.tex <==
\begin{tabular}{@{}l r r r r r r@{}}
\toprule
Model + Harness & Chemistry (24) & Physics (22) & Life Sciences (21) & Math \& CS (11) & Materials Science (9) & Engineering (6) \\
\midrule
GPT-6.2 Astra + Codex & \textbf{59.8} & \textbf{71.0} & \textbf{54.5} & \textbf{59.9} & \textbf{74.2} & \textbf{74.7} \\
GPT-6.2 Sol + Codex & 55.5 & 58.9 & 53.0 & 58.4 & 67.0 & 73.7 \\
Qwen4-Max + Qoder & 45.8 & 41.3 & 42.4 & 42.2 & 60.2 & 47.1 \\
Kimi K3.1 Pro + Kimi Code & 35.1 & 44.5 & 38.8 & 42.7 & 55.5 & 54.7 \\
HY4 + DSH & 30.6 & 38.9 & 39.1 & 31.3 & 53.7 & 48.6 \\
DeepSeek V4.1 Flash 1017 + DSH & 26.8 & 33.2 & 35.0 & 26.0 & 49.3 & 50.4 \\
HY4 + CodeBuddy & 18.2 & 34.2 & 30.4 & 18.6 & 48.2 & 36.8 \\
GLM 5.3 + ZCode & 19.5 & 25.9 & 22.5 & 18.7 & 40.9 & 34.8 \\
HY4 Flash + CodeBuddy & 16.0 & 27.2 & 23.6 & 20.7 & 36.3 & 38.2 \\
MiMo V2.6 Pro + MiMo Code & 9.5 & 25.2 & 18.0 & 24.7 & 39.3 & 28.9 \\
Doubao Seed 2.1 Pro + TRAE & 17.7 & 23.9 & 17.9 & 14.2 & 39.2 & 24.9 \\
\midrule
\textit{11-entrant mean} & 30.4 & 38.6 & 34.1 & 32.5 & 51.3 & 46.6 \\
\bottomrule
\end{tabular}


==> generated/tab_groupmatrix_zh.tex <==
\begin{tabular}{@{}l r r r r r r@{}}
\toprule
Model + Harness 组合 & 化学 (24) & 物理学 (22) & 生命科学 (21) & 数学与计算机 (11) & 材料科学 (9) & 工程科学 (6) \\
\midrule
GPT-6.2 Astra + Codex & \textbf{59.8} & \textbf{71.0} & \textbf{54.5} & \textbf{59.9} & \textbf{74.2} & \textbf{74.7} \\
GPT-6.2 Sol + Codex & 55.5 & 58.9 & 53.0 & 58.4 & 67.0 & 73.7 \\
Qwen4-Max + Qoder & 45.8 & 41.3 & 42.4 & 42.2 & 60.2 & 47.1 \\
Kimi K3.1 Pro + Kimi Code & 35.1 & 44.5 & 38.8 & 42.7 & 55.5 & 54.7 \\
HY4 + DSH & 30.6 & 38.9 & 39.1 & 31.3 & 53.7 & 48.6 \\
DeepSeek V4.1 Flash 1017 + DSH & 26.8 & 33.2 & 35.0 & 26.0 & 49.3 & 50.4 \\
HY4 + CodeBuddy & 18.2 & 34.2 & 30.4 & 18.6 & 48.2 & 36.8 \\
GLM 5.3 + ZCode & 19.5 & 25.9 & 22.5 & 18.7 & 40.9 & 34.8 \\
HY4 Flash + CodeBuddy & 16.0 & 27.2 & 23.6 & 20.7 & 36.3 & 38.2 \\
MiMo V2.6 Pro + MiMo Code & 9.5 & 25.2 & 18.0 & 24.7 & 39.3 & 28.9 \\
Doubao Seed 2.1 Pro + TRAE & 17.7 & 23.9 & 17.9 & 14.2 & 39.2 & 24.9 \\
\midrule
\textit{11 组均值} & 30.4 & 38.6 & 34.1 & 32.5 & 51.3 & 46.6 \\
\bottomrule
\end{tabular}


==> generated/tab_groupperf_zh.tex <==
\begin{tabularx}{\linewidth}{@{}l r r >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X l@{}}
\toprule
学科大类 & 题数 & 11组均分 & 第 1 名（均分） & 第 2 名（均分） & 头部差与 95\% 区间 \\
\midrule
化学 & 24 & 30.4 & GPT-6.2 Astra (59.8) & GPT-6.2 Sol (55.5) & $+4.3$ $[-7.4, +15.7]$ \\
物理学 & 22 & 38.6 & GPT-6.2 Astra (71.0) & GPT-6.2 Sol (58.9) & $+12.1$ $[+5.8, +19.5]$（已分出） \\
生命科学 & 21 & 34.1 & GPT-6.2 Astra (54.5) & GPT-6.2 Sol (53.0) & $+1.4$ $[-10.9, +13.5]$ \\
数学与计算机 & 11 & 32.5 & GPT-6.2 Astra (59.9) & GPT-6.2 Sol (58.4) & $+1.5$ $[-1.8, +5.3]$ \\
材料科学 & 9 & 51.3 & GPT-6.2 Astra (74.2) & GPT-6.2 Sol (67.0) & $+7.3$ $[+0.6, +14.3]$（已分出） \\
工程科学 & 6 & 46.6 & GPT-6.2 Astra (74.7) & GPT-6.2 Sol (73.7) & $+1.0$ $[+0.1, +2.2]$（已分出） \\
地球科学 * & 1 & 61.2 & GPT-6.2 Astra (100.0) & GPT-6.2 Sol (100.0) & — \\
\bottomrule
\end{tabularx}


==> generated/tab_outcomes_zh.tex <==
\begin{tabular}{@{}l r r r@{}}
\toprule
研究任务标签 & 覆盖题数 & 受影响单元 / 总单元 & 至少一次超时或异常比例 \\
\midrule
靶点选择性 & 5 & 33 / 55 & 60.0\% \\
分子设计 & 6 & 35 / 66 & 53.0\% \\
构型优化 & 5 & 28 / 55 & 50.9\% \\
机制分析 & 6 & 24 / 66 & 36.4\% \\
路线评估 & 12 & 36 / 132 & 27.3\% \\
合成路线设计 & 11 & 29 / 121 & 24.0\% \\
细胞状态分析 & 5 & 11 / 55 & 20.0\% \\
\bottomrule
\end{tabular}


==> generated/tab_pairs_zh.tex <==
\begin{tabular}{@{}lrrrrl@{}}
\toprule
配对比较 & 共同题 & 分差 & 95\% 区间 & 胜 / 负 & 主要信号 \\
\midrule
HY4：DSH $-$ CodeBuddy & 65 & $+11.0$ & $[+6.7, +15.4]$ & 42 / 10 & Harness 效应（显著） \\
DSH：HY4 $-$ DeepSeek V4.1 Flash 1017 & 65 & $+6.0$ & $[+1.5, +10.5]$ & 36 / 16 & 同 Harness 换模型（显著） \\
CodeBuddy：HY4 $-$ HY4 Flash & 65 & $+5.1$ & $[+0.7, +9.7]$ & 32 / 13 & 模型规格换代（显著） \\
GPT-6.2：Astra $-$ Sol & 65 & $+5.2$ & $[+0.0, +10.5]$ & 28 / 10 & 同代变体差异 \\
\bottomrule
\end{tabular}


==> generated/tab_rank_zh.tex <==
\begin{tabular}{@{}r l r c r r r r r r r@{}}
\toprule
\# & Model + Harness 组合 & 均分 & 95\% 区间 & pass@1 & pass@5 & pass\textsuperscript{5} & 超时/异常 & 用时 & 输出Tok & 效率 \\
\midrule
1 & \modellogo{gpt}GPT-6.2 Astra + Codex & \textbf{61.3} & [51.3, 70.6] & 55.7\% & 60.0\% & 49.2\% & 4.9\% & 42m & 105k & 4.97 \\
2 & \modellogo{gpt}GPT-6.2 Sol + Codex & \textbf{56.0} & [46.8, 65.1] & 46.2\% & 53.8\% & 36.9\% & 3.1\% & 35m & 126k & 3.68 \\
3 & \modellogo{qwen}Qwen4-Max + Qoder & 44.0 & [35.1, 52.8] & 33.2\% & 49.2\% & 20.0\% & 12.4\% & 176m & 201k & 1.25 \\
4 & \modellogo{kimi}Kimi K3.1 Pro + Kimi Code & 40.5 & [32.1, 48.8] & 29.5\% & 50.8\% & 15.4\% & 8.6\% & 150m & 217k & 1.11 \\
5 & \modellogo{hy4}HY4 + DSH & 38.3 & [30.0, 46.9] & 24.3\% & 44.6\% & 10.8\% & 6.2\% & 148m & 216k & 1.29 \\
6 & \modellogo{deepseek}DeepSeek V4.1 Flash 1017 + DSH & 32.3 & [25.1, 39.9] & 17.8\% & 40.0\% & 4.6\% & 8.2\% & 191m & 228k & 0.88 \\
7 & \modellogo{hy4}HY4 + CodeBuddy & 27.3 & [20.5, 34.8] & 15.1\% & 29.2\% & 4.6\% & 14.9\% & 172m & 291k & 1.17 \\
8 & \modellogo{glm}GLM 5.3 + ZCode & 23.9 & [17.5, 30.5] & 15.4\% & 36.9\% & 3.1\% & 32.3\% & 300m & 211k & 0.90 \\
9 & \modellogo{hy4}HY4 Flash + CodeBuddy & 22.2 & [16.5, 28.4] & 9.8\% & 21.5\% & 1.5\% & 5.2\% & 114m & 107k & 1.17 \\
10 & \modellogo{mimo}MiMo V2.6 Pro + MiMo Code & 20.5 & [14.2, 27.1] & 9.2\% & 16.9\% & 4.6\% & 13.6\% & 159m & 167k & 1.03 \\
11 & \modellogo{doubao}Doubao Seed 2.1 Pro + TRAE & 19.8 & [14.1, 26.1] & 10.8\% & 24.6\% & 1.5\% & 37.5\% & 300m & 160k & 0.51 \\
\bottomrule
\end{tabular}


==> generated/tab_typematrix_zh.tex <==
\begin{tabular}{@{}l r r r r r@{}}
\toprule
Model + Harness 组合 & 数值仿真 (15) & 开放设计 (23) & 多阶段分析 (16) & 工具规划 (11) & 总均分 (65) \\
\midrule
\modellogo{gpt}GPT-6.2 Astra + Codex & \textbf{87.3} & \textbf{71.6} & 40.4 & 34.5 & \textbf{61.3} \\
\modellogo{gpt}GPT-6.2 Sol + Codex & 73.3 & 61.1 & \textbf{46.2} & 36.4 & 56.0 \\
\modellogo{qwen}Qwen4-Max + Qoder & 60.6 & 37.2 & 39.6 & \textbf{41.8} & 44.0 \\
\modellogo{kimi}Kimi K3.1 Pro + Kimi Code & 55.8 & 44.6 & 33.1 & 21.8 & 40.5 \\
\modellogo{hy4}HY4 + DSH & 67.2 & 31.8 & 38.1 & 12.7 & 38.3 \\
\modellogo{deepseek}DeepSeek V4.1 Flash 1017 + DSH & 53.4 & 32.9 & 27.8 & 9.1 & 32.3 \\
\modellogo{hy4}HY4 + CodeBuddy & 50.5 & 22.6 & 30.9 & 0.0 & 27.3 \\
\modellogo{glm}GLM 5.3 + ZCode & 42.5 & 19.2 & 20.9 & 12.7 & 23.9 \\
\modellogo{hy4}HY4 Flash + CodeBuddy & 34.2 & 24.9 & 22.4 & 0.0 & 22.2 \\
\modellogo{mimo}MiMo V2.6 Pro + MiMo Code & 41.7 & 17.1 & 19.6 & 0.0 & 20.5 \\
\modellogo{doubao}Doubao Seed 2.1 Pro + TRAE & 29.1 & 15.3 & 21.2 & 14.5 & 19.8 \\
\bottomrule
\end{tabular}


==> sections/en/06_limitations.tex <==
\section{Limitations}\label{sec:limitations}

Clearly delineating evaluation boundaries is essential to scientific credibility. DeltaScience v1.0 currently carries five limitations:
\begin{itemize}
\item \textbf{Uneven disciplinary coverage.} The \DSNumTasks{} tasks in v1.0 reflect initial contributing teams; areas such as Earth Science remain sparse, and several of the \DSNumSubfields{} subfields contain only 1--2 tasks.
\item \textbf{Reference-value uncertainty.} Scientific reference fields (such as EFIT++ reconstructions in FUS-0001) carry domain-specific measurement or modeling uncertainty, which is documented per task.
\item \textbf{Five-trial bounds on rare events.} Five trials cleanly separate never-solved from reliably solved tasks, but confidence intervals for low-probability passes or rare timeouts remain wide.
\item \textbf{Contamination risks on public examples.} Public case-study documentation may enter future pretraining corpora; the core suite therefore remains strictly private and rotates monthly.
\item \textbf{Extrapolation boundary.} Task scores measure deliverable quality under pinned computational environments and must not be equated directly with wet-lab validation or full R\&D productivity.
\end{itemize}

